Local inversion of maps: A new attack on Symmetric encryption, RSA and ECDLP

This paper presents algorithms for local inversion of maps and shows how several important computational problems such as cryptanalysis of symmetric encryption algorithms, RSA algorithm and solving the elliptic curve discrete log problem (ECDLP) can be addressed as local inversion problems. The methodology is termed as the \emph{Local Inversion Attack}. It utilizes the concept of \emph{Linear Complexity} (LC) of a recurrence sequence generated by the map defined by the cryptanalysis problem and the given data. It is shown that when the LC of the recurrence is bounded by a bound of polynomial order in the bit length of the input to the map, the local inversion can be accomplished in polynomial time. Hence an incomplete local inversion algorithm which searches a solution within a specified bound on computation can estimate the density of weak cases of cryptanalysis defined by such data causing low LC. Such cases can happen accidentally but cannot be avoided in practice and are fatal insecurity flaws of cryptographic primitives which are wrongly assumed to be secure on the basis of exponential average case complexity. An incomplete algorithm is proposed for solving problems such as key recovery of symmetric encryption algorithms, decryption of RSA ciphertext without factoring the modulus, decrypting any ciphertext of RSA given one plaintext ciphertext pair created with same public key in chosen ciphertext attack and solving the discrete logarithm on elliptic curves over finite fields (ECDLP) as local inversion problems. It is shown that when the LCs of the respective recurrences for given data are small, solutions of these problems are possible in practically feasible time and memory resources.

==> deleted.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Introduction

An objective of Cryptanalysis is to estimate efforts (in time, memory and complexity) required to subvert a functionality of cryptographic algorithms (or primititves). A cryptanalysis problem usually translates to determining the unknown information (such as symmetric or private keys) given the ciphertext corresponding to a known information or a publicly known output. Since the unknown has finite length in information bits, a brute force search of the unknown is always one option to solve any cryptanalysis problem. However cryptographic primitives are designed to have large enough lengths of private and symmetric keys which render brute force result in exponential complexity. However even with advanced algebraic methods cryptanalysis of algorithms such as AES128 continue to require exponential complexity. Attacks on RSA by factorization of the modulus have resulted into estimating sub-exponential complexity for cryptanalysis of RSA which do not weaken RSA at realistic scales. The elliptic curve discrete log problem (ECDLP) on the other hand has no known methods better than exponential complexity. Hence all of these primitives which have dominant role in practical cryptography are assumed to be secure. Point is what gurantees there are no exceptional or accidental weak instances (or sessions) of these primitives? The attack we propose in this paper based on local inversion of maps in finite fields, allows determining such weak encryptions in these primitives.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{strofsolns}
Given an arbitrary point $y$ in $\ftwo^n$ solutions of $F(x)=y$ are described by following possibilities
\begin{enumerate}
    \item $F(x)=y$ has no solution iff $y$ belongs to the GOE of $F$.
    \item $F(x)=y$ has solution in a periodic orbit $P$ iff $y$ belongs to $P$. Such a periodic orbit is unique. Given $y$ in a periodic orbit $P$ and the unique solution to $F(x)=y$ in $P$, all other possible solutions belong to the chains $f^{k}(z),k\geq 1$ for $z$ in the GOE of $F$. 
    \item If $y$ is neither in a periodic orbit nor in the GOE, then all solutions to $F(x)=y$ arise in some of the chains $F^{(k)}(z),k\geq 1$ for $z$ in the GOE. 
\end{enumerate}
\end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}\label{Embeddingsolver}
\caption{Incomplete algorithm to find the unique solution of an embedding}
\begin{algorithmic}[1]
\State\textbf{Input}: $F:\ff^n\rightarrow\ff^m$, $n-m=t$, $y$ in $\ff^n$, $M$ an upper bound of polynomial order $O(n^r)$.
\State\textbf{Output}: One solution of $F(x)=y$ if one exists otherwise returns that there is no conclusion.
\Procedure{Solution}{$y=F(x)$}
\State Compute the projection equations (\ref{projectioneqns}) for $i=1,2,\ldots,(t+1)$.
\State Compute the sequence $S(F_1,y(1))=\{F_1^{(k)}(y(1))\}$ for $k=0,1,\ldots,M$.
\State Set $m=\lfloor M/2\rfloor$.
\Repeat
\State Compute matrices $H(m)$, $H(m+1)$ (as shown in (\ref{hankelmatrix})) for $S(F_1,y(1))$.
\State Compute $\rank H(m)$, $\rank H(m+1)$.
\While{
\[
m=\rank H(m)=\rank H(m+1)=m
\]
}
\State Compute the minimal polynomial co-efficients $\hat{\alpha}$ in (\ref{Hankeleqn}).
\State Compute solution $x(1)$ as in (\ref{solution}).
\If {$(F_i(x)=y(i)\forall i=1,2,\ldots,(t+1)$}
\State $x:=x(1)$
\State \% Verification to avoid false positive solutions.
\State Return: Solution $x$.
\EndIf
\EndWhile
\If{$\rank H(m)<\rank H(m+1)$}
\State Return: No conclusion within the bound $M$, ($\mbox{LC}>\lfloor M/2\rfloor$).
\EndIf
\If{$\rank H(m)=\rank H(m+1)<m$}
\State $m\leftarrow m-1$.
\EndIf
\Until{$m=1$}
\State Return: No conclusion within the bound $M$, ($\mbox{LC}>\lfloor M/2\rfloor$).
\EndProcedure
\end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
